Near Real-Time Social Distance Estimation in London

During the COVID-19 pandemic, policy makers at the Greater London Authority, the regional governance body of London, UK, are reliant upon prompt and accurate data sources. Large well-defined heterogeneous compositions of activity throughout the city are sometimes difficult to acquire, yet are a necessity in order to learn 'busyness' and consequently make safe policy decisions. One component of our project within this space is to utilise existing infrastructure to estimate social distancing adherence by the general public. Our method enables near immediate sampling and contextualisation of activity and physical distancing on the streets of London via live traffic camera feeds. We introduce a framework for inspecting and improving upon existing methods, whilst also describing its active deployment on over 900 real-time feeds.

==> bibliography_removed.tex <==
@Inproceedings{deutscher_automatic_2002,
	address = {Berlin, Heidelberg},
	title = {Automatic {Camera} {Calibration} from a {Single} {Manhattan} {Image}},
	isbn = {978-3-540-47979-6},
	abstract = {We present a completely automatic method for obtaining the approximate calibration of a camera (alignment to a world frame and focal length) from a single image of an unknown scene, provided only that the scene satisfies a Manhattan world assumption. This assumption states that the imaged scene contains three orthogonal, dominant directions, and is often satisfied by outdoor or indoor views of man-made structures and environments.},
	booktitle = {Computer {Vision} — {ECCV} 2002},
	publisher = {Springer Berlin Heidelberg},
	author = {Deutscher, J. and Isard, M. and MacCormick, J.},
	editor = {Heyden, Anders and Sparr, Gunnar and Nielsen, Mads and Johansen, Peter},
	year = {2002},
	pages = {175--188}
}

@article{glaister, title={85.13 Least squares revisited}, volume={85}, DOI={10.2307/3620485}, number={502}, journal={The Mathematical Gazette}, publisher={Cambridge University Press}, author={Glaister, P.}, year={2001}, pages={104–107}}

@misc{hamelijnck2019multiresolution,
    title={Multi-resolution Multi-task Gaussian Processes},
    author={Oliver Hamelijnck and Theodoros Damoulas and Kangrui Wang and Mark Girolami},
    year={2019},
    eprint={1906.08344},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@INPROCEEDINGS{redmon2016yolo9000,  author={Redmon, Joseph and Farhadi, Ali},  booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},   title={YOLO9000: Better, Faster, Stronger},   year={2017},  volume={},  number={},  pages={6517-6525},  doi={10.1109/CVPR.2017.690}}

@INPROCEEDINGS{choi2019gaussian,
  author={Choi, Jiwoong and Chun, Dayoung and Kim, Hyun and Lee, Hyuk-Jae},
  booktitle={2019 IEEE/CVF International Conference on Computer Vision (ICCV)}, 
  title={Gaussian YOLOv3: An Accurate and Fast Object Detector Using Localization Uncertainty for Autonomous Driving}, 
  year={2019},
  volume={},
  number={},
  pages={502-511},
  doi={10.1109/ICCV.2019.00059}}
  
 @misc{impact3,
  author = {{Lloyd’s Register Foundation}},
  title = {{Understanding London's busyness during COVID-19}},
  howpublished = "\url{https://www.lrfoundation.org.uk/en/news/understanding-londons-busyness/}",
  year = {2021}, 
  note = "[Online; accessed 16-Oct-2021]"
}
